A Novel Approach to Model the Kinematics of Human Fingers Based on an Elliptic Multi-Joint Configuration

In this paper, we present a novel kinematic model of the human phalanges based on the elliptical motion of their joints. The presence of the soft elastic tissues and the general anatomical structure of the hand joints highly affect the relative movement of the bones. Commonly used assumption of circular trajectories simplifies the designing process but leads to divergence with the actual hand behavior. The advantages of the proposed model are demonstrated through the comparison with the conventional revolute joint model. Conducted simulations and experiments validate designed forward and inverse kinematic algorithms. Obtained results show a high performance of the model in mimicking the human fingertip motion trajectory.

==> Human_Finger_Anatomy.tex <==
Human index finger has a complex structure in anatomy, understanding the component, shape, attach point and function of index finger will be helpful in developing a bionic robot finger.

1) Index finger bones: Fig. \ref{fig: Bones_Joints}(a) shows that the index finger constitutes four bones: distal phalanx, intermediate phalanx, proximal phalanx and metacarpal bones. These four bones form the structure of index finger and also offer the attachment points for muscle, ligaments and joint capsule. The distal phalanx is flat on palmar side and has a concave articular surface base. The intermediate phalanx, proximal phalanx and metacarpal bone all have the head with convex articular surface and the base with concave articular surface. The concave and convex surfaces are coordinate to determine the rotation in specific orientation. The intermediate phalanx and proximal phalanx have one direction curved surface, which is from dorsal side to palmar side. The metacarpal bone has an additional curved surface which is from radial side to ulnar side.

2) Index finger joints: Finger joints, containing the articular capsule and ligaments, are responsible for connecting the bones and supporting movements. Fig. \ref{fig: Bones_Joints}(b) shows that the index finger comprises four joints, The Distal Interphalangeal Joint (DIP), which is formed by the base of the distal phalanx and head of the intermediate phalanx. Proximal Interphalangeal Joint (PIP Joint), which is formed by the base of intermediate phalanx and the head of proximal phalanx. Metacarpophalangeal Joint (MCP joint), which is formed by the base of the proximal phalanx and the head of metacarpal bone. Carpometacarpal Joint (CMC Joint), which is formed by the base of the metacarpal bone and the trapezoid (one of the carpals). The CMC joint of index finger is immobile, so we will mainly focus on the previous three joints. 

3) Index articular capsule: The joints have two types soft tissue: The articular capsule and ligaments. The function of articular capsule is for containing the synovial fluid and supporting the ligaments. Fig. \ref{fig: Capsule_ligaments}(a) shows the structure of articular capsule,  It's composed of the synovial layer and the fibrous layer. Synovial layer consists of fibrous tissue (capsular ligaments). It attaches firmly with the head and base of bones, it also can support the synovial layer. The synovial layer is a highly vascularised layer for absorbing and secreting synovial fluid. Synovial fluid is a non-Newtonian fluid. It's for lubrication and absorbing shock\cite{quinn_2018_structures}. 

4) Index finger ligaments: The ligaments have important function for the movement of finger. It provides the passive limitation and restriction to the bones. The ligaments are flexible and soft when they are slack, and has very large strength when being pulled. It's really difficult to define how many ligaments that the index finger has, because they are not independent, which have multiple connections with each other. We will introduce the main ligaments of the index finger Fig. \ref{fig: Capsule_ligaments}(b). i) Palmar Plate, it arises respectively from the base of distal phalanx, intermediate phalanx and  proximal phalanx, inserts on the intermediate phalanx, proximal phalanx and metacarpal phalanx by two check-rein ligaments (Fig. \ref{fig: checkrein}). It enhance the stability of DIP, PIP and MCP joint, it's responsible for limiting the hyperextension. ii) Collateral ligament consists of the proper ligament and the accessory collateral ligament. The proper ligament arises respectively from the radial or ulnar side of the head of metacarpal bone, proximal phalanx and intermediate phalanx, inserts on the base of proximal phalanx, intermediate phalanx and distal phalanx. The collateral ligament is oblique, it will be taut during the flexion of finger and slack during the extension of finger. iii) Accessory collateral ligament is found in PIP and DIP joints. It arises farther proximal and palmar on the head of  metacarpal bone, proximal phalanx and intermediate phalanx, it inserts on the palmar plate. It's slack during flexion and taut during extension\cite{bernhardhirt_2017_hand}. iv) Extensor hood, the extensor hood is a complex structure consists of central slip, lateral bands and other soft tissue\ref{fig: extensor hood}. The central slip connects with the extensor digitorum communis. The lateral bands connect with lumbrical muscle and interosseus muscle. The function of extensor hood is flexing the MCP joint and extend the PIP and DIP joints at same time. 

5) The muscle of index finger: There are seven muscles which drive the index finger: first palmar interosseus, first dorsal interosseus, first lumbrical, extensor indicis, extensor digitorum, flexor digitorum profundus and flexor digitorum superficialis
\begin{figure*}[!ht]
\centering
\includegraphics[scale=0.6]{Images/Bones_Joints.png}
\caption{Bones and joints of index finger. (a) The name and position of bones. (b) The name and position of joints\cite{villarreal_2007_english}.}
\label{fig: Bones_Joints}
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[scale=0.7]{Images/capsule_ligaments.png}
\caption{Articular capsule and ligaments of finger. (a) The structure of capsule. (b) The ligaments of finger (palmar side)\cite{schuenke_2020_general}.}
\label{fig: Capsule_ligaments}
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[scale=0.7]{Images/checkrein.png}
\caption{Volar plate of finger joint\cite{salihangin_2020_comparative}.}
\label{fig: checkrein}
\end{figure*}

\begin{figure*}[!ht]
\centering
\includegraphics[scale=0.7]{Images/extensorhood.PNG}
\caption{Extensor hood of finger\cite{bernhardhirt_2017_hand}}
\label{fig: extensor hood}
\end{figure*}

==> Sections/Methods.tex <==
\begin{algorithm}[H]
\title{IK_Analytical}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  \KwInput{
  $T\in {{\mathbb{R}}^{3\times n}}\text{ }T=[{{\overline{f}}_{1,}}{{\overline{f}}_{2}}...{{\overline{f}}_{n}}]\text{ };{{\overline{f}}_{n}}={{[f_{x}^{n},f_{y}^{n},f_{z}^{n}]}^{T}}$\;
  $\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }\text{ }para\in {{\mathbb{R}}^{1\times 12}}$
  }
  \KwOutput{
  $\hat{\theta }\in {{\mathbb{R}}^{4\times n}}\text{ }\hat{\theta }={{\left[ {{{\hat{\theta }}}_{1}},{{{\hat{\theta }}}_{2}},{{{\hat{\theta }}}_{3}},{{{\hat{\theta }}}_{4}} \right]}^{T}}$
  $\text{ }{{\hat{\theta }}_{i}}=[\theta _{i}^{1},...\theta _{i}^{n}]\in {{\mathbb{R}}^{1\times n}}\text{ }i\in \left[ 1...4 \right]$
}

% Set Function Names
  \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{$NonlinearFunction\_Solver$}
  \SetKwFunction{FSub}{Sub}
 
% Write Function with word ``Function''
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FSum{$F(\theta )$, $\theta$}}{
    Using non-linear optimization method to do the\;iterations of $\vartriangle \theta =pinv(J(F(\theta )))F(\theta )$ until the\;error ($\vartriangle e=F(\theta )-0$) smaller smaller we need.
    \KwRet $\theta$\;
  }
% Set Function Names
  \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{$theta1\_calculate$}
  \SetKwFunction{FSub}{Sub}
 
% Write Function with word ``Function''
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FSum{$T$, $para$}}{
        from $T$ and $para$ calculate equation ${{F}_{1}}({{\hat{\theta }}_{1}})$\;
        %This function is to calculate the first angle of\;Ab/Ad movement according to fingertip position.\;Then we do the loop the calculation to get all angles ($\hat{\theta }_{1}$) for n points.\;
        This function is to calculate the first angle of\;Ab/Ad movement according to fingertip position.
        
    \KwRet $\hat{\theta }_{1}$\;
  }
% Set Function Names
  \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{$theta234\_calculate$}
  \SetKwFunction{FSub}{Sub}
 
% Write Function with word ``Function''
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FSum{$T$, $para$,$\hat{\theta }_{1}$}}{
        Substitute $\hat{\theta }_{1}$ into $\hat{\theta }$  Get $\overline{f}_{n}$ from $T$\;
        Set initial value of $\theta _{2}^{i},\theta _{3}^{i},\theta _{4}^{i}$ and using\;$NonlinearFunction\_Solver$ to calculate the angle\;on each fingertip point and centralized storage to\; $theta\in {{\mathbb{R}}^{3\times n}}$, and we have $\hat{\theta}=[\hat{\theta}_{1},theta]$\;
    \KwRet $\hat{\theta }$
  }
$\hat{\theta_{1}}=theta1\_calculate(T,para)$\;
$\hat{\theta}=theta234\_calculate(T,para,\hat{\theta_{1}})$\;
save $\hat{\theta}$
\caption{The IK of Analytical Solution}
\end{algorithm}


==> Sections/Methods/Moment_Ellipse.tex <==
The moment arm of elliptical joint is various during the movement of joint, which causes different moment (with constant force). Assuming an external force $\vec{F}={{\left[ {{F}_{x}}\text{ }{{F}_{y}}\text{ }{{F}_{z}} \right]}^{T}}$ acts on fingertip. The moment on each joint is: 
\begin{equation}
    \tau =-{{J}^{T}}\vec{F}\text{ }\text{ }\text{ }J=\frac{\partial \bar{q}(\theta )}{\partial \theta }
\end{equation}
$\tau ={{[{{\tau }_{1}}\text{ }{{\tau }_{2}}\text{ }{{\tau }_{3}}\text{ }{{\tau }_{4}}]}^{T}}$ is the moment of joint from Ab/Ad of MCP joint to F/E of DIP joint. ${\bar{q}(\theta )}$ is taken from $\bar{q}_{0}$ of equation (12), which is the function of $\theta$ and also is the coordinate of fingertip under coordinate frame $0$.

==> Sections/Related_Work/ACT.tex <==
The Anatomically Correct Testbed hand (ACT hand) is developed by Ashish D. Deshpande, ZheXu et al. It's the first hybrid rigid-soft robotic hand trying to mimic soft tissue corresponding to the real human hand. Fig. \ref{fig: relatedwork} (a) shows the structure of ACT hand. It mimicked the tissue on dorsal side of three fingers: middle finger, index finger and thumb, they also developed a mechanism of wrist, avoiding the movement of wrist  affecting three fingers. This hand was able to do some simple grasping. In their experiment, they selected 9 objects commonly used in daily life and then picked them up with an ACT hand. 

ACT hand is a great inspiration for us, but it is not perfect。 First of all, the joint part still needs the support of hard materials. Although the human bone model is used, the connection between the bones is still a hard connection. The essence of the joint is a conventional revolute joint. The soft tissue on the dorsal side only plays a role in dispersing the tension of the tendons, but does not stabilize the joints.


Our robotic hand has used soft connections between the bones, using only ligaments and joint capsules to connect these bones. This allows the hand to have better compliance which will improve the grip performance. 


\begin{figure*}[!ht]
\centering
\includegraphics[scale=0.6]{Images/Relatedwork1.png}
\caption{The Prototypes of Hybrid Rigid-Soft Robotic Hand: (a) ACT Hand\cite{ACT}   (b) Highly Biomimetic Anthropomorphic Robotic Hand\cite{Washington}}
\label{fig: relatedwork}
\end{figure*}

==> Sections/Related_Work/Design.tex <==
Nowadays, the research on hybrid rigid-soft biomimetic robotic hand has just started. There are only several prototypes. The difficulties in developing this type of prototype is that the human hand mechanism is very complicated, it is difficult to mimic the structure, and also the soft connection tissue of robotic hand brings control problems. However, there are still two good prototypes that we will present and analyze them.

==> Sections/Related_Work/Washingtonhand.tex <==
The highly biomimetic anthropomorphic robotic hand is developed by Zhe Xu and Emanuel Todorov. This hand has a high level of completion. This hand mimicked five fingers like human hand (no wrist). It used the bone model of human hand and the connections between the bones are made of soft materials, the connection points of these soft tissue refers to the human hand. The structure of the hand on dorsal side is relatively exquisite, mimicking the structure of the human hand extensor hood to a high degree. This structure is very similar to the human hand in terms of shape and connection points, these structures have been proved in their experiments that they also have similar functions to the same parts of human hand extensor hood. In addition, in their follow-up experiments, they let robotic hand used different grasping modes (power grasp and precision grasp) to prove that the hand has good grasping ability and versatility.
